Powerful Design of Small Vision Transformer on CIFAR10

Vision Transformers (ViTs) have demonstrated remarkable success on large-scale datasets, but their performance on smaller datasets often falls short of convolutional neural networks (CNNs). This paper explores the design and optimization of Tiny ViTs for small datasets, using CIFAR-10 as a benchmark. We systematically evaluate the impact of data augmentation, patch token initialization, low-rank compression, and multi-class token strategies on model performance. Our experiments reveal that low-rank compression of queries in Multi-Head Latent Attention (MLA) incurs minimal performance loss, indicating redundancy in ViTs. Additionally, introducing multiple CLS tokens improves global representation capacity, boosting accuracy. These findings provide a comprehensive framework for optimizing Tiny ViTs, offering practical insights for efficient and effective designs. Code is available at https://github.com/erow/PoorViTs.

==> sec/4_experiment.tex <==
\section{Experiment}

\subsection{Tiny Vision Transformer}

\paragraph{Baseline.}
The baseline code is based on \cite{gani2022train}. Many data augmentation methods are applied, including CutMix~\citep{yun2019cutmix}, MixUp~\citep{zhang2017mixup}, AutoAugment (aa)~\citep{hoffer2020augment}, and Repeated Augment\citep{cubuk2019autoaugment,hoffer2020augment}. Additionally, regularization methods include label smoothing~\citep{Szegedy_2016_CVPR}, stochastic depth~\citep{huang2016deep}, and random erasing~\citep{zhong2020random}. All models by default are trained for 100 epochs with a batch size of 256 on a single NVIDIA 3090 GPU paired with an AMD EPYC 7532 32-Core Processor. The Adam optimizer is used with a cosine schedule with learning rate of 0.002, which is decayed using a cosine scheduling strategy with a warmup of 10 epochs. The weight decay rate is 5e-2. The tiny vision transformer has 12 heads in attention, 9 transformer blocks, and 64 patches for images (patch size is 4x4). The experimental results are summarized in \cref{tab:exps}.


\paragraph{Profiler.}
To understand the training bottleneck, we employ the PyTorch Profiler~\citep{pytorchPyTorchProfiler}. \cref{fig:profile} visualizes the time span of each procedure by tracing\footnote{\url{edge://tracing/} in Edge browser.}.  The backward process consumes the most training time. Therefore, the bottleneck of training ViTs is the high cost of dealing with large feature maps during forward and backward. \cref{tab:benchmark_tinyvit} compares the forward time with different batch sizes. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{pics/profile.png}
    \caption{Tracing one training step. One step (120.7 ms) involves forward (25.2 ms), backward (79.3 ms), optimization(12.7 ms), and others. }
    \label{fig:profile}
\end{figure}

\begin{table}[ht]
    \centering
    \resizebox{0.8\textwidth}{!}{%
    \begin{tabular}{c|cccccc}
        \toprule
        \textbf{Batch Size (bs)} & \textbf{32} & \textbf{64} & \textbf{128} & \textbf{256} & \textbf{512} & \textbf{1024} \\ 
        \midrule
        \textbf{Throughput (images/s)} & 3162.09 & 6521.61 & 9449.16 & 9721.13 & 10368.24 & 10607.06 \\ 
        \textbf{Memory Usage (GB)} & 0.31 & 0.62 & 1.25 & 2.50 & 5.00 & 9.98 \\ 
        \bottomrule
    \end{tabular}%
    }
    \caption{Benchmark of Tiny ViT on an NVIDIA RTX 3090 GPU. }
    \label{tab:benchmark_tinyvit}
\end{table}


\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccccccc}
        \toprule
        & \textbf{Baseline} & \multicolumn{3}{c}{\textbf{Augmentation}} & \multicolumn{2}{c}{\textbf{patch}} & \multicolumn{5}{c}{\textbf{MLA}} & \multicolumn{3}{c}{\textbf{DDP}} \\
        \cmidrule(r){3-5} \cmidrule(r){6-7} \cmidrule(r){8-12} \cmidrule(r){13-15}
        &          & -aa   & -mixup & -cutmix & sin   & Witen   & qkv   & kv   & qk   & q    & k    & bs256 &       bs1024 &\\
        \midrule
        \textbf{Runtime} & 4658     & 4684  & 4656   & 4651   & 4687  & 4676  & 4805 & 4756 & 4785 & 4716 & 4711 & 3582  &       1371 & 1545\\
        \textbf{Val/Acc} & 93.65    & 92.14 & 93.68  & 92.77  & 93.43 & 93.28 & 91.8 & 92.43 & 92.42 & 93.32 & 92.5 & 93.44 &    92.09& 92.38\\
        \bottomrule
    \end{tabular}}
    \caption{Summary of our experiments. `aa' denotes AutoAugment. Data augmentation is critical except Mixup. The learnable position embeddings demonstrate the best performance. Compressing queries during training exhibits the less performance drop. Increasing batch size reduces the training time when distributed data parallel is applied, while, diminishing performance. Lion~\citep{chen2023lion} is more effective than AdamW~\citep{loshchilov2019adamw} to optimize the tiny ViT.}
    \label{tab:exps}
\end{table}

\subsection{[...]}

\paragraph{Augmentation.}  
The experiments demonstrate the significance of data augmentation methods in improving validation accuracy. Removing AutoAugment (`-aa') results in a noticeable drop in accuracy (92.14 vs. 93.65), highlighting its importance. Similarly, disabling CutMix (`-cutmix') leads to a decline (92.77 vs. 93.65). Interestingly, removing MixUp (`-mixup`) marginally improves accuracy (93.68), suggesting it may not be as beneficial in this setup. These results underline the importance of selecting appropriate augmentations tailored to the dataset and architecture.

\paragraph{Patch Toekn Initialization.}  
We utilize learnable positional embeddings by default. The positional embeddings can be alternated by sinusoidal positional embeddings (`sin`) which is non-learnable and fixed during training. Sinusoidal embeddings achieve slightly worse validation accuracy (93.43 vs. 93.65).
We follow \citeauthor{ysam-code_cifar} to initialize the patch embedding instead of random initialization. The whitening initialization (`Witen`) finds the patterns in the dataset as illustrated in \cref{fig:whitening} to speed up the training process. However, this technique, working well in CNN, does not apply to ViTs.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{pics/white.png}
    \caption{Whitening patterns in patch embedding.}
    \label{fig:whitening}
\end{figure}






\paragraph{Distributed Data Parallel (DDP).}  
We conduct distributed data parallel training with 4 3090 GPUs. Experiments with DDP show that increasing the batch size reduces the training time significantly (e.g., from 3582s to 1371s with `bs1024`). However, larger batch sizes lead to diminish validation accuracy (92.09 vs. 93.65 for `bs256`). This trade-off emphasizes the need to balance computational efficiency with model performance when scaling training. 


\paragraph{Optimizer.}  
The Lion optimizer~\citep{chen2023lion} is compared against AdamW~\citep{loshchilov2019adamw} for optimizing the Tiny ViT. \cref{fig:opt} compares Lion to Adam for finding a good solution. Lion achieves a higher accuracy (92.38), demonstrating its superior capability for this architecture.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{pics/opt.png}
    \caption{Accuracy over training time with lion optimizer. Although Lion consumes more time for each step, it requires fewer iterations to find a good solution.}
    \label{fig:opt}
\end{figure}


\subsection{Low-dimensional Patch Tokens}

\paragraph{Low-Rank Compression.}  
Different configurations of Multi-Head Latent Attention (MLA)~\citep{liu2024deepseek} were evaluated, including modifications to the queries (`q'), keys (`k'), or values (`v'). Compressing all three (`qkv`) incurs a noticeable performance drop (91.8 vs. 93.65), while modifications targeting specific combinations (e.g., `kv', `qk', `q', and `k') yield better results. In particular, there is a marginal drop in precision when compressing `q', matching the results in \cite{liu2024deepseek}. These findings indicate the potential for low-rank compression in ViTs to reduce activation memory.


\paragraph{Multi-Class Token.}
We investigate the potential solution to improve efficiency for ViTs. One natural idea is to reduce the dimension of tokens. However, a low-dimension token means less capacity for visual information, which can be observed in \cref{tab:tokens} where the accuracy drops 3.24\% by reducing the dimension to 96. We argue that patch tokens overwhelming in number (64 vs. 1) have higher capacity than the CLS token. Even though patch tokens could represent the image perfectly, these semantic representations are difficult to be expressed by a narrow CLS token. To prove this hypothesis, we introduce more CLS tokens to capture the global representation. These CLS tokens will be concatenated and fed to the classifier. Our simple multi-class token (MCLS) strategy boots the capacity of global representation effectively. \cref{tab:tokens} proves our hypothesis by using 2 CLS tokens to improve accuracy from 90.41 to 93.95. 
Note that, our MCLS is significantly different to the Mctformer+\citep{xu2024mctformer+} in which the class information is distributed to several CLS tokens. In contrast, our proposal is a simple way of expanding the dimension of the CLS token, and each CLS token denotes partial of the real CLS token.

\begin{table}[]
    \centering
\begin{tabular}{c|ccc}
\toprule
   dim  &  192 & 96 & 96\\
   num CLS & 1 &   1   & 2 \\
   
   \midrule
  acc & 93.65 & 90.41&  93.95 \\
  
  \bottomrule
  \end{tabular}
\caption{Multi class token}
\label{tab:tokens}
\end{table}
